Vision Transformer Adapters for Generalizable Multitask Learning

We introduce the first multitasking vision transformer adapters that learn generalizable task affinities which can be applied to novel tasks and domains. Integrated into an off-the-shelf vision transformer backbone, our adapters can simultaneously solve multiple dense vision tasks in a parameter-efficient manner, unlike existing multitasking transformers that are parametrically expensive. In contrast to concurrent methods, we do not require retraining or fine-tuning whenever a new task or domain is added. We introduce a task-adapted attention mechanism within our adapter framework that combines gradient-based task similarities with attention-based ones. The learned task affinities generalize to the following settings: zero-shot task transfer, unsupervised domain adaptation, and generalization without fine-tuning to novel domains. We demonstrate that our approach outperforms not only the existing convolutional neural network-based multitasking methods but also the vision transformer-based ones. Our project page is at \url{https://ivrl.github.io/VTAGML}.

==> main/images/teaser.tex <==

\begin{center}
\centering
{\includegraphics[height= 5.5cm, width=17.3cm ]{AVTaR/figures/teaser.png}}
%\vspace{-11.3 pt}
\setlength{\abovecaptionskip}{0pt}
\captionof{figure}{ Our AVTaR model that leverages a vision adapter atop a pre-trained transformer backbone decreases computational requirement by over an order of magnitude w.r.t the baselines, while outperforming both the single-task~\cite{unet} and multi-task baselines ~\cite{MulT,tawt,Vandenhende_2021,xtam}. We apply AVTaR to three settings, from left to right, multi-task learning (on Vkitti2 benchmark), zero-shot task transfer setting (on the Synthia benchmark) and unsupervised domain adaptation setting (for Vkitti2$\rightarrow$Cityscapes), respectively. All models shown here are trained on the segmentation and depth labels (\textit{'S-D'}). For zero-shot task transfer here, surface normal estimation is the zero-shot task. Best seen on screen and when zoomed within the yellow circled regions.
}\label{fig:teaser}\vspace{-10pt}
\end{center}
